PORT: Preference Optimization on Reasoning Traces

Preference optimization methods have been successfully applied to improve not only the alignment of large language models (LLMs) with human values, but also specific natural language tasks such as summarization and stylistic continuations. This paper proposes using preference optimization methods on Chain-of-Thought steps in order to improve the mathematical reasoning performances of language models. While the chosen answers are obtained from datasets that include reasoning traces, we propose two complementary schemes for generating rejected answers: weak LLM prompting, and digit corruption. Our approach leads to increased accuracy on the GSM8K and AQuA-RAT mathematical reasoning benchmarks for Falcon2-11B and Mistral-7B. Additionally, the improved abilities transfer to non-mathematical tasks, including the ARC benchmark and symbolic reasoning challenges. For example, our method can lead to up to relative 8.47% and 18.73% increases in accuracy on the GSM8K and AQuA benchmarks respectively, without any extra annotations. This work suggests that the path towards better language reasoning abilities goes through spending resources on creating high-quality datasets of reasoning traces.

==> removesection.tex <==
\section{REMOVESECTION ! Additional results}
\begin{table}[h]
        \centering
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA & ARC \\
                \midrule
                Base model &  $54.66$ & $21.65$ & $49.91$  \\
                SFT (1 epoch) & $54.66$ & $20.87$ & $49.91$  \\
                SFT & $55.43$ & $21.26$ & $49.74$  \\
                SFT (5 epochs) & $54.66$ & $19.69$ & $49.66$\\
                \bottomrule
            \end{tabular}
        \caption{Accuracy (in percentage) of the SFT on the three considered tasks.The base model here is Falcon2-11B.\label{tab:base_vs_sft_epochs}}
\end{table}

\begin{table}[!h]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                %
                %\multirow{3}{*}{Iteration 0} & SPIN & $49.23$ & $32.97$ & $65.90$ & $18.73$ & $72.22$ & $41.06$ & $46.69$  \\
                Base model (Falcon2-11B) &  $54.66$ & $21.65$ & $49.91$  \\
                \midrule
                %\multirow{3}{*}{Iteration 1} & SPIN & $49.32$ & $33.19$ & $66.46$ & $21.00$ & $73.06$ & $40.89$ & $47.32$  \\
                SFT & $\textbf{55.43}$ & $21.26$ & $49.74$  \\
                SFT-(with $<< >>$) & $54.66$ & $\textbf{22.05}$ & $49.91$  \\
                \midrule                
            \end{tabular}
            \end{minipage}
            }
        
        \caption{Accuracy (in percentage) finetune with effect of the calcualtion symbol on GSM8K.}
%\end{wraptable}
\end{table}

\begin{table}[]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                %
                %\multirow{3}{*}{Iteration 0} & SPIN & $49.23$ & $32.97$ & $65.90$ & $18.73$ & $72.22$ & $41.06$ & $46.69$  \\
                Base model (Falcon2-11B) &  $54.66$ & $21.65$ & $49.91$  \\
                \midrule
                %\multirow{3}{*}{Iteration 1} & SPIN & $49.32$ & $33.19$ & $66.46$ & $21.00$ & $73.06$ & $40.89$ & $47.32$  \\
                SFT & $55.43$ & $21.26$ & $49.74$  \\
                DPO-llama-7b-corrupted-3epochs-$\beta=0.1$ &  $49.51$ & $21.26$  & $50.94$  \\
                \midrule
                %\multirow{3}{*}{\shortstack[l]{Iteration 2}} & SPIN & $50.34$ & $33.91$ & $67.01$ & $20.24$ & $73.82$ & $40.65$ & $47.66$  \\
                DPO-llama-7b-corrupted-1epochs-$\beta=0.1$ &  $52.84$ & $19.69$ & $51.02$  \\
                DPO-llama-7b-corrupted-1epochs-$\beta=0.2$ &  $56.10$ & $19.29$ & $50.60$  \\
                DPO-llama-7b-corrupted-1epochs-$\beta=0.3$ &  $55.19$ & $19.29$ & $50.77$  \\
                DPO-llama-7b-corrupted-1epochs-$\beta=0.5$ &  $56.03$ & $20.08$ & $50.94$  \\
                \bottomrule
            \end{tabular}
            \end{minipage}
            }
        
        \caption{hyperparameer search - beta - here 1 epoch only. DPO learning rates here are $8 \times 10^{-6}$ + best hyperparams on unccorupted llama}
%\end{wraptable}
\end{table}

\begin{table}[]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                %
                %\multirow{3}{*}{Iteration 0} & SPIN & $49.23$ & $32.97$ & $65.90$ & $18.73$ & $72.22$ & $41.06$ & $46.69$  \\
                Base model (Falcon2-11B) &  $54.66$ & $21.65$ & $49.91$  \\
                \midrule
                %\multirow{3}{*}{Iteration 1} & SPIN & $49.32$ & $33.19$ & $66.46$ & $21.00$ & $73.06$ & $40.89$ & $47.32$  \\
                SFT & $55.43$ & $21.26$ & $49.74$  \\
                DPO-llama-7b-corrupted-3epochs-$\beta=0.1$ &  $49.51$ & $21.26$  & $50.94$  \\
                \midrule
                %\multirow{3}{*}{\shortstack[l]{Iteration 2}} & SPIN & $50.34$ & $33.91$ & $67.01$ & $20.24$ & $73.82$ & $40.65$ & $47.66$  \\
                DPO-llama-7b-corrupted-3epochs-$\beta=0.2$ &  $53.3$ & $20.08$ & $50.94$  \\
                DPO-llama-7b-corrupted-2epochs-$\beta=0.2$ &  $54.74$ & $20.98$ & $50.94$  \\
                DPO-llama-7b-corrupted-1epochs-$\beta=0.2$ &  $56.10$ & $19.29$ & $50.60$  \\
                \bottomrule
            \end{tabular}
            \end{minipage}
            }
        
        \caption{hyperparameer search - n epochs - here DPO learning rates here are $8 \times 10^{-6}$}
%\end{wraptable}
\end{table}

\begin{table}[]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                %
                %\multirow{3}{*}{Iteration 0} & SPIN & $49.23$ & $32.97$ & $65.90$ & $18.73$ & $72.22$ & $41.06$ & $46.69$  \\
                Base model (Falcon2-11B) &  $54.66$ & $21.65$ & $49.91$  \\
                \midrule
                %\multirow{3}{*}{Iteration 1} & SPIN & $49.32$ & $33.19$ & $66.46$ & $21.00$ & $73.06$ & $40.89$ & $47.32$  \\
                SFT & $55.43$ & $21.26$ & $49.74$  \\
                \midrule
                %\multirow{3}{*}{\shortstack[l]{Iteration 2}} & SPIN & $50.34$ & $33.91$ & $67.01$ & $20.24$ & $73.82$ & $40.65$ & $47.66$  \\
                DPO-llama-7b-corrupted-1epochs-$\beta=0.2$-$LR=8\times 10^{-4}$ &  $55.57$ & $20.87$ & $52.56$  \\
                DPO-llama-7b-corrupted-1epochs-$\beta=0.2$-$LR=8\times 10^{-7}$ &  $54.81$ & $23.23$ & $49.66$  \\
                DPO-llama-7b-corrupted-1epochs-$\beta=0.2$-$LR=8\times 10^{-6}$ &  $56.10$ & $19.29$ & $50.60$  \\
                DPO-llama-7b-corrupted-2epochs-$\beta=0.2$-$LR=8\times 10^{-6}$ &  $54.74$ & $20.98$ & $50.94$  \\
                DPO-llama-7b-corrupted-1epochs-$\beta=0.2$-$LR=1\times 10^{-8}$ &  $54.74$ & $23.62$ & $49.74$  \\
                DPO-llama-7b-corrupted-2epochs-$\beta=0.2$-$LR=1\times 10^{-8}$ &  $55.04$ & $24.41$ & $49.91$  \\
                \bottomrule
            \end{tabular}
            \end{minipage}
            }
        
        \caption{hyperparameer search - lr and n epochs}
%\end{wraptable}
\end{table}

\begin{table}[h]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                %
                %\multirow{3}{*}{Iteration 0} & SPIN & $49.23$ & $32.97$ & $65.90$ & $18.73$ & $72.22$ & $41.06$ & $46.69$  \\
                Base model (Falcon2-11B) &  $54.66$ & $21.65$ & $49.91$  \\
                \midrule
                %\multirow{3}{*}{Iteration 1} & SPIN & $49.32$ & $33.19$ & $66.46$ & $21.00$ & $73.06$ & $40.89$ & $47.32$  \\
                SFT ( 1 epoch) & $54.66$ & $20.87$ & $49.91$  \\
                SFT & $55.43$ & $21.26$ & $49.74$  \\
                SFT (5 epochs) & $54.66$ & $19.69$ & $49.66$\\
                \midrule
                %\multirow{3}{*}{\shortstack[l]{Iteration 2}} & SPIN & $50.34$ & $33.91$ & $67.01$ & $20.24$ & $73.82$ & $40.65$ & $47.66$  \\
                \textbf{ours} \\
                
                DPO-digit corruption &  $\mathbf{58.30}$ \scriptsize{\textcolor{teal}{+3.64}} & $19.96$ & $50.77$  \\
                KTO-digit corruption &  $40.26$ & $17.72$ & $51.62$  \\
                DPO-gemma-2b-it & $48.45$ & $21.26$ & $52.13$  \\
                DPO-llama-7b-chat &  $47.08$ & $\mathbf{23.62}$ \scriptsize{\textcolor{teal}{+1.97}} & $52.47$  \\
                DPO-\{digit corruption + gemma-2b-it\} &  $40.79$ & $21.26$ & $52.82$  \\
                DPO-\{digit corruption + llama-7b-chat\}  & $44.88$ & $21.26$ & $\mathbf{52.99}$ \scriptsize{\textcolor{teal}{+3.08}}  \\
                DPO-\{gemma-2b-it + llama-7b-chat\}  & $45.72$ & $22.05$ & $52.73$  \\
                \bottomrule
            \end{tabular}
            \end{minipage}
            }
        
        \caption{Accuracy (in percentage) of the different models on the three considered tasks -- with old hyperprameters and wrong eval protocol. The different DPO fine-tuned models differ in how the rejected answers are generated.}
%\end{wraptable}
\end{table}

\subsection*{best hyperparameters}
\begin{table}[h]
        \centering
        
        \resizebox{\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                Base model (Falcon2-11B)&  $54.66$ & $31.50$ & $76.11$  \\
                \midrule
                SFT & $55.43$ & $30.71$ & $75.60$   \\
                \midrule
                \textbf{ours} \\
                % DPO-gemma-2b-it   & $53.68$ & $29.92$ & $75.94$  \\
                DPO-gemma-2b-it x3 & $51.40$ & $35.04$ & $76.45$  \\
                % DPO-llama-7b corrupted &  $56.10$ & $30.71$ & $77.05$  \\
                
                DPO-llama-7b corrupted x3 & $54.51$ & $29.53$ & $76.19$ \\
                DPO-llama-7b corrupted + digit & $56.56$ & $32.68$ & $77.47$ \\
                DPO-llama-7b corrupted + digit x3 & $56.48$ & $30.31$ & $77.73$ \\
                % DPO-iterative-corrupted & $55.65$ & $33.46$ & $76.28$ \\
                DPO-digit-corruption-x3 &  $59.29$ & $33.07$ & $76.79$  \\
                DPO-digit-corruption-x1 &  $58.91$ & $35.04$ & $76.02$  \\
                \bottomrule
            \end{tabular}
            \end{minipage}
            }
        \caption{Accuracy (in percentage) with best hyperparams\label{tab:h12}}
\end{table}

\begin{table}[]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                %
                %\multirow{3}{*}{Iteration 0} & SPIN & $49.23$ & $32.97$ & $65.90$ & $18.73$ & $72.22$ & $41.06$ & $46.69$  \\
                Base model (Falcon2-11B) &  $54.66$ & $21.65$ & $49.91$  \\
                \midrule
                %\multirow{3}{*}{Iteration 1} & SPIN & $49.32$ & $33.19$ & $66.46$ & $21.00$ & $73.06$ & $40.89$ & $47.32$  \\
                SFT & $55.43$ & $21.26$ & $49.74$  \\
                DPO-gemma-2b-it & $48.45$ & $21.26$ & $52.13$  \\
                DPO-corrupted-iterative &  $23.65$ & $21.26$ & $51.28$ \\ 
                DPO-llama-7b-chat &  $47.08$ & $\mathbf{23.62}$ & $52.47$  \\
                \midrule
                %\multirow{3}{*}{\shortstack[l]{Iteration 2}} & SPIN & $50.34$ & $33.91$ & $67.01$ & $20.24$ & $73.82$ & $40.65$ & $47.66$  \\
                DPO-gemma-2b-it-$\beta=0.2$-1epoch & $53.6$ & $20.87$ & $51.79$  \\        DPO-corrupted-iterative-$\beta=0.2$-1epoch &  $55.65$ & $20.47$ & $51.28$  \\ 
                DPO-llama-7b-chat-$\beta=0.2$-1epoch &  $53.45$ & $22.05$ & $51.71$  \\
                \bottomrule
            \end{tabular}
            \end{minipage}
            }
        
        \caption{additional results}
%\end{wraptable}
\end{table}

\subsection*{ORPO hyperparameter search}

For ORPO, starting from the base model (not the SFT one obviously) - with digit corrupted answers - results on GSM8K only:
\begin{itemize}
    \item $\beta=0.001$, $LR=1\times 10^{-8}$, 1 epoch: 55.42
    \item $\beta=0.001$, $LR=8\times 10^{-8}$, 1 epoch: 54.89
    \item $\beta=0.005$, $LR=1\times 10^{-8}$, 1 epoch: 55.12
    \item $\beta=0.01$, $LR=1\times 10^{-8}$, 1 epoch: 54.89
    \item $\beta=0.01$, $LR=8\times 10^{-8}$, 1 epoch: 54.73
    \item $\beta=0.01$, $LR=8\times 10^{-6}$, 1 epoch: 42.38
    \item $\beta=0.1$, $LR=8\times 10^{-6}$, 1 epoch: 40.40
    \item $\beta=0.1$, $LR=8\times 10^{-6}$, 3 epochs: 20.54
    \item $\beta=0.1$, $LR=8\times 10^{-6}$, 5 epochs: 14.32
    \item $\beta=0.2$, $LR=8\times 10^{-6}$, 1 epoch: 38.28    
    \item $\beta=0.5$, $LR=8\times 10^{-6}$, 1 epoch: 35.7    
\end{itemize}

\subsection{MISTRAL results on GSM8K}


mistral7b-base0.1: 38.51\\
SFT-finetuned-3epochs-GSM8K: 39.12\\
DPO-llm-only-1-llamacorrupted-besthyperparams-$\beta=0.5$: 41.69\\
DPO-corr-only-1-besthyperparams-$\beta=0.5$: 42.68\\
DPO-corr-only-3-besthyperparams-$\beta=0.5$: 42.76\\
DPO-corr-llm-1-llamacorrupted-besthyperparams-$\beta=0.5$: 40.03 \\

\subsection*{Noisy preference labels}
taking DPO-llama7b-corrupted-1epochs-$\beta=0.2$ as a baseline, which achieves $56.10$ percent accuracy in GSM8K.
\begin{itemize}
    \item cDPO-llama-7b-corrupted-$\beta=0.2$-1epochs-0.01 smoothing : $55.34$
    \item cDPO-llama-7b-corrupted-$\beta=0.2$-1epochs-0.1 smoothing : $53.29$
    \item cDPO-llama-7b-corrupted-$\beta=0.2$-1epochs-0.01 smoothing : $6.14$
    \item RDPO-llama-7b-corrupted-$\beta=0.2$-1epochs-0.1 smoothing : $16.98$
\end{itemize}

\section*{additional results - digit corruption}

\begin{table}[]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                %
                %\multirow{3}{*}{Iteration 0} & SPIN & $49.23$ & $32.97$ & $65.90$ & $18.73$ & $72.22$ & $41.06$ & $46.69$  \\
                Base model (Falcon2-11B) &  $54.66$ & $21.65$ & $49.91$  \\
                \midrule
                %\multirow{3}{*}{Iteration 1} & SPIN & $49.32$ & $33.19$ & $66.46$ & $21.00$ & $73.06$ & $40.89$ & $47.32$  \\
                SFT & $55.43$ & $21.26$ & $49.74$  \\
                \midrule
                %\multirow{3}{*}{\shortstack[l]{Iteration 2}} & SPIN & $50.34$ & $33.91$ & $67.01$ & $20.24$ & $73.82$ & $40.65$ & $47.66$  \\
                DPO-digit-corruption-x3-1epochs-$\beta=0.2$ &  $59.29$ & $20.08$ & $50.26$  \\
                DPO-digit-corruption-x1-1epochs-$\beta=0.2$ &  $58.91$ & $19.29$ & $50.68$  \\
                DPO-digit-corruption-x1-1epochs-$\beta=0.5$ &  $57.47$ & $20.47$ & $50.85$  \\
                \bottomrule
            \end{tabular}
            \end{minipage}
            }
        
        \caption{additional results}
%\end{wraptable}
\end{table}

\subsection*{Compare predicting  remaining reasoning steps VS only next step}
\begin{table}[!h]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                %
                %\multirow{3}{*}{Iteration 0} & SPIN & $49.23$ & $32.97$ & $65.90$ & $18.73$ & $72.22$ & $41.06$ & $46.69$  \\
                Base model (Falcon2-11B) &  $54.66$ & $21.65$ & $49.91$  \\
                \midrule
                %\multirow{3}{*}{Iteration 1} & SPIN & $49.32$ & $33.19$ & $66.46$ & $21.00$ & $73.06$ & $40.89$ & $47.32$  \\
                SFT & ${55.43}$ & $\textbf{21.26}$ & $49.74$  \\
                SFT-remaining & $54.81$ & $20.87$ & $50.17$  \\
                \midrule
                %\multirow{3}{*}{\shortstack[l]{Iteration 2}} & SPIN & $50.34$ & $33.91$ & $67.01$ & $20.24$ & $73.82$ & $40.65$ & $47.66$  \\
                \textbf{ours} \\
                
                DPO-digit corruption &  $\mathbf{58.30}$ & $19.96$ & $\textbf{50.77}$  \\
                DPO-digit corruption - remaining &  $57.01$ & $19.96$ & $50.09$  \\
                
            \end{tabular}
            \end{minipage}
            }
        
        \caption{Accuracy (in percentage) finetune with predicting only next step vs the remaining reasoning step}
%\end{wraptable}
\end{table}

\subsection*{SFT \& DPO -- Effect of \textit{prompt with \underline{math-related} few-shots}}
\begin{table}[!h]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                %
                %\multirow{3}{*}{Iteration 0} & SPIN & $49.23$ & $32.97$ & $65.90$ & $18.73$ & $72.22$ & $41.06$ & $46.69$  \\
                Base model (Falcon2-11B) &  $54.66$ & $..$ & $..$  \\
                \midrule
                %\multirow{3}{*}{Iteration 1} & SPIN & $49.32$ & $33.19$ & $66.46$ & $21.00$ & $73.06$ & $40.89$ & $47.32$  \\
                SFT & $55.43$ & $28.74$ & $70.41$  \\
                SFT-(3-few-shot) & $55.95$ & $\textbf{21.65}$ & $49.57$  \\
                \midrule
                DPO-digit corruption &  $\mathbf{58.30}$ & $19.96$ & ${50.77}$  \\
                DPO-digit corruption - (3-few-shot) &  $50.11$ & $20.47$ & $\textbf{51.79}$  \\
                
            \end{tabular}
            \end{minipage}
            }
        
        \caption{Accuracy (in percentage) impact of the few-shot prompting}
\vspace*{-7mm}
%\end{wraptable}
\end{table}


\section*{SFT -- Effect of training dataset}
\begin{table}[!h]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                %
                %\multirow{3}{*}{Iteration 0} & SPIN & $49.23$ & $32.97$ & $65.90$ & $18.73$ & $72.22$ & $41.06$ & $46.69$  \\
                Base model (Falcon2-11B) &  $54.66$ & $31.50$ & $76.11$  \\
                \midrule
                %\multirow{3}{*}{Iteration 1} & SPIN & $49.32$ & $33.19$ & $66.46$ & $21.00$ & $73.06$ & $40.89$ & $47.32$  \\
                SFT on GSM8K & $55.43$ & $30.71$ & $75.60$   \\
                SFT on AQuA & $54.89$ & $31.50$ & $75.68$  \\
                SFT on AQuA+GSM8K & $54.89$ & $30.71$ & $76.54$  \\
                SFT on AQuA+GSM8K (1 epoch only) & $53.45$ & $33.86$ & $75.60$  \\
                \midrule                
            \end{tabular}
            \end{minipage}
            }
        
        \caption{Accuracy (in percentage) -- effect of training dataset}
%\end{wraptable}
\end{table}





\section*{Finetuned with AQUA -- SFT \& DPO}
\begin{table}[!h]
%\begin{wraptable}{l}{11cm}
        \centering
        
        \resizebox{.95\linewidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{llllcccc}
                \toprule
                \textbf{Model} & GSM8K & AQuA-RAT & ARC (hard) \\
                \midrule
                Base model (Falcon2-11B) &  $54.66$ & $31.50$ & $76.11$  \\
                \midrule
                SFT on AQUA & $54.89$ & $31.50$ & $75.68$\\
                \midrule
                DPO--digit corruption & $57.70$ & $37.40$ & $76.88$  \\
                DPO--digit corruption x 3 & $54.51$ & $34.25$ & $77.05$  \\
                DPO--llama7B corrupted & $55.57$ & $33.86$ & $76.71$  \\
                DPO--{llama7B + digit} corruption & $57.85$ & $31.50$ & $77.05$  \\
                DPO--{llama7B + digit} corruption x3 & $54.51$ & $34.25$ & $76.62$  \\
                \midrule                
            \end{tabular}
            \end{minipage}
            }
        
        \caption{Accuracy (in percentage) -- effect of training and DPO finetuning  with AQUA dataset}
%\end{wraptable}
\end{table}
